Improving Discrete Latent Representations With Differentiable Approximation Bridges

Modern neural network training relies on piece-wise (sub-)differentiable functions in order to use backpropagation to update model parameters. In this work, we introduce a novel method to allow simple non-differentiable functions at intermediary layers of deep neural networks. We do so by training with a differentiable approximation bridge (DAB) neural network which approximates the non-differentiable forward function and provides gradient updates during backpropagation. We present strong empirical results (performing over 600 experiments) in four different domains: unsupervised (image) representation learning, variational (image) density estimation, image classification, and sequence sorting to demonstrate that our proposed method improves state of the art performance. We demonstrate that training with DAB aided discrete non-differentiable functions improves image reconstruction quality and posterior linear separability by 10% against the Gumbel-Softmax relaxed estimator [37, 26] as well as providing a 9% improvement in the test variational lower bound in comparison to the state of the art RELAX [16] discrete estimator. We also observe an accuracy improvement of 77% in neural sequence sorting and a 25% improvement against the straight-through estimator [5] in an image classification setting. The DAB network is not used for inference and expands the class of functions that are usable in neural networks.

==> Preliminaries.tex <==
\section{Preliminaries}

In their seminal work \cite{robbins1951stochastic}, Robbins and Monroe
developed a framework of optimization to solve for the minimum of a
function $[\mathbb{E}[G(\theta_t)] - C]$, under the assumption of the
existence of a unique solution. They characterized the iterative update rule as:
% \vskip -0.2in
\begin{align}
  \theta_{t+1} = \theta_t - \alpha_t [\mathbb{E}[G(\theta_t)] - C]. \label{robbins_monroe}
\end{align}

Given an observable random variable $G$, parametrized by $\theta_t$,
the objective is defined as solving for $\mathbb{E}[G(\theta_t)] - C$,
wherein $C$ is some constant.  If we assume that the gradient of $\mathbb{E}[G]$ is $K$-Lipschitz
continuous, we can replace $\mathbb{E}[G]$ with its gradient, $\mathbb{E}[\nabla G]$; this is due to the
fact that we can bound the difference between iterative updates of
$\theta_t$ with and without the application of $\mathbb{E}[G]$ (derives from the
Lipschitz property):
% \vskip -0.2in
\begin{align}
  || \mathbb{E}[\nabla G(\theta_{t})] - \mathbb{E}[\nabla G(\theta_{t-1})] ||_2 \leq K
  ||\theta_{t} - \theta_{t-1} ||_2. \label{grad_diff}
\end{align}

Given that we can lower bound the normed-parameter difference (right
hand side of Equation \ref{grad_diff}) by the
normed-functional gradients (left hand size of Equation $\ref{grad_diff}$) and through the assumption of small
iterates in parameter space ($K < 1$), repeated application of the
update rule in Equation \ref{robbins_monroe} converges to a
fixed point (in expectation). This derives from the Banach Fixed Point Theorem that
states:

\newmdtheoremenv{theo}{Theorem}
\begin{theo}
  Given a metric space $(\theta, d)$ and a contractive
  mapping $F: \theta \mapsto \theta$, then  $F$ admits a
  unique fixed point $\theta^* \in \theta$.
\end{theo}\label{banach_theorem}

In the specific case of Equation \ref{grad_diff}, the metric
$d$ is the L2-norm. Note, a norm is a more rigid constraint than a metric since norms require
translation invariance and the scaling property in addition to all the
requirements of a metric. This simplified analysis demonstrates that
in the case of convex functions, SGD reaches a fixed point which
incidentally also happens to be the global minima. In the case of non-convex functions, no such
guarantee can be made and SGD can only be shown to reach a local
minima / fixed point. In either case, the convergence properties are strongly tied
to the smooth K-Lipschitz properties of the function $G$.

Since non-differentiable functions do not possess the smooth,
K-Lipschitz gradient discussed above, we introduce an auxiliary DAB
neural network model and couple it with a regularizer described in the
next section. The objective of the regularizer (implemented under a
Gaussianity assumption) is to provide a smooth, continuous
approximation to the non-differentiable function. During forward pass
(at both training and inference), the model uses the
non-differentiable function's output in subsequent layers, however during the
backward pass, the gradient from the DAB network is used to update the
model. We experimented with training the DAB network apriori and simply using it
to relay back gradients (rather than training both
objectives jointly), but did not notice a quantitative difference and
only report our findings on the latter.

% In the specific case of $G$ and its gradient $\nabla G$, the metric
% $d$ is the L2-norm as specified in Equation \ref{grad_diff}. Note that
% a norm is a more rigid constraint than a metric since norms require
% translation invance and the scaling property in addition to the
% requirements of a metric.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

